A Variational Framework for the Thermomechanics of Gradient-Extended Dissipative Solids -- with Applications to Diffusion, Damage and Plasticity

The paper presents a versatile framework for solids which undergo nonisothermal processes with irreversibly changing microstructure at large strains. It outlines rate-type and incremental variational principles for the full thermomechanical coupling in gradient-extended dissipative materials. It is shown that these principles yield as Euler equations essentially the macro- and micro-balances as well as the energy equation. Starting point is the incorporation of the entropy and entropy rate as canonical arguments into constitutive energy and dissipation functions, which additionally depend on the gradient-extended mechanical state and its rate, respectively. By means of (generalized) Legendre transformations, extended variational principles with thermal as well as mechanical driving forces can be constructed. On the thermal side, a rigorous distinction between the quantity conjugate to the entropy and the quantity conjugate to the entropy rate is essential here. Formulations with mechanical driving forces are especially suitable when considering possibly temperature-dependent threshold mechanisms. With regard to variationally consistent incrementations, we suggest an update scheme which renders the exact form of the intrinsic dissipation and is highly suitable when considering adiabatic processes. It is shown that this proposed numerical algorithm has the structure of an operator split. To underline the broad applicability of the proposed framework, we set up three model problems as applications: Cahn-Hilliard diffusion coupled with temperature evolution, where we propose a new variational principle in terms of the species flux vector, as well as thermomechanics of gradient damage and gradient plasticity. In a numerical example we study the formation of a cross shear band.

==> examples/shearband/contour/fig.tex <==
\begin{figure}%         don't change
%
\hspace{-0.9cm}
%  \footnotesize
  \psfrag{aa}     [cc][cc] {{\footnotesize a)}}
  \psfrag{bb}     [cc][cc] {{\footnotesize b)}}
  \psfrag{cc}     [cc][cc] {{\footnotesize c)}}
  \psfrag{dd}     [cc][cc] {{\footnotesize d)}}
  \psfrag{ee}     [cc][cc] {{\footnotesize e)}}
  \psfrag{ff}     [cc][cc] {{\footnotesize f)}}
  \psfrag{amax}    [ll][ll] {{\footnotesize  2.3}}
  \psfrag{amin}    [ll][l] {{\footnotesize  0.0}}
  \psfrag{tmax}    [ll][ll] {{\footnotesize  472}}
  \psfrag{tmin}    [ll][ll] {{\footnotesize  293}}
  \psfrag{al}    [ll][ll] {{\footnotesize  $\alpha$}}
  \psfrag{th}    [ll][ll] {{\footnotesize  $\theta$~[K]}}
  \includegraphics*[scale=0.6]{fig.eps}
\caption {Cross Shear Localization. Contour plots of equivalent plastic strain $\alpha$ and temperature $\theta$ at final displacement $\bar u = 5$~mm for a discretization of one quarter of the specimen by $20 \times 40$ finite elements. The chosen plastic length scale parameters are a), d) $l=0.05$~mm; b), e) $l=0.1$~mm and c), f) $l=0.2$~mm.  
}
\label{\LABEL}%         don't change
\end{figure}%         don't change


==> examples/shearband/force-disp/fig.tex <==
\begin{figure}%         don't change
%
\centering
{
  \psfrag{iso}      [ll][ll] {\scriptsize{isothermal}}
  \psfrag{11}       [ll][ll] {\scriptsize{$15 \times 30$ el.}}
  \psfrag{22}       [ll][ll] {\scriptsize{$20 \times 40$ el.}}
  \psfrag{33}       [ll][ll] {\scriptsize{$25 \times 50$ el.}}
  \psfrag{0}       [cc][cc] {\scriptsize{0}}
  \psfrag{0.5}       [cc][cc] {\scriptsize{0.5}}
  \psfrag{1}       [cc][cc] {\scriptsize{1}}
  \psfrag{1.5}       [cc][cc] {\scriptsize{1.5}}
  \psfrag{2}       [cc][cc] {\scriptsize{2}}
  \psfrag{2.5}       [cc][cc] {\scriptsize{2.5}}
  \psfrag{3}       [cc][cc] {\scriptsize{3}}
  \psfrag{4}       [cc][cc] {\scriptsize{4}}
  \psfrag{5}       [cc][cc] {\scriptsize{5}}
  \psfrag{10}       [cc][cc] {\scriptsize{10}}
  \psfrag{15}       [cc][cc] {\scriptsize{15}}
  \psfrag{20}       [cc][cc] {\scriptsize{20}}
  \psfrag{25}       [cc][cc] {\scriptsize{25}}
  \psfrag{30}       [cc][cc] {\scriptsize{30}}
  \psfrag{x}        [cc][cc] {\scriptsize{displacement $\bar u$ [mm]}}
  \psfrag{y}        [cc][cc] {\scriptsize{load $F$ [kN]}}
  \psfrag{aa}       [cc][cc] {\footnotesize{a)}}
  \psfrag{bb}       [cc][cc] {\footnotesize{b)}}

  \includegraphics*[scale=0.6]{fig.eps}
}
\caption {Cross Shear Localization. Load-deflection curves. a) Mesh dependent structural response for local theory with $l=0$~mm and b) mesh objective response for gradient theory with $l=0.1$~mm. The dashed line in b) shows the behavior of the specimen under isothermal condition and one observes the influence of thermal softening on the yield stress according to \req{cshear_2}$_2$. Note, that in b) the final displacement is $\bar u = 5$~mm, whereas in a) it is $\bar u = 2.5$~mm.
}
\label{\LABEL}%         don't change
\end{figure}%         don't change


==> examples/shearband/tab01.tex <==
\begin{table}
  \centering
%  \footnotesize
  \caption{Parameters of representative numerical example.}
%  \label{\LABEL}
%  \label{table1}
%   \vspace*{0.2cm}
%   \begin{tabular}{|crrrr|}
%   \hline
    \begin{tabular}{lrrrr}
    No.& Parameter & Name & Value& Unit \\ \hline
    1 & $\kappa$       & bulk modulus  & $164.2$ &kN/mm$^2$\\
    2 & $\mu$          & shear modulus &  $80.2$& kN/mm$^2$\\
    3 & $l $      & plastic length scale & $\{0.05,0.1,0.2  \}$& mm \\
    4 & $\alpha_T$            & thermal expansion coefficient& $10^{-5}$& 1/K\\
    5 & $C$            & heat capacity & $3.588 \cdot 10^{-3}$& kN/(mm$^2$K)\\
    6 & $k$            & heat conduction coefficient & $0.0$& kN/(sK)\\
    7 & $\theta_0$           & reference temperature & $293.0$& K\\
    8 & $h_0$       & initial hardening parameter &$-0.13$ &kN/mm$^2$ \\
    9 & $y_0$       & initial yield stress &$0.45$&kN/mm$^2$ \\
    10 & $w_h$       & thermal softening coefficient &$0.0$&1/K \\
    11 & $w_0$       & thermal softening coefficient &$0.002$&1/K \\
    12 & $\eta_f$       & viscosity parameter  &$10^{-6}$&kNs/mm$^2$ \\
    \hline
  \end{tabular}
\label{\LABEL}
\end{table}



==> floats/fields/fig.tex <==
\begin{figure}%         don't change

\centering
{
%
  \footnotesize
  \psfrag{t}     [r][r]     {$ \BP \,  \Bn_0 \!\ni\!\bar \Bt$}
  \psfrag{QQ}    [r][r]     {$\Bq\!\cdot\! \Bn_0 \!=\!\bar q$}
  \psfrag{HH}    [r][r]     {$\BH^l \,  \Bn_0 \!\ni\! \Bzero$}
  \psfrag{n}     [lt][lt]   {$\Bn_0$}
  \psfrag{x}     [c][c]     {$\BX\in\calB$}
  \psfrag{phi}   [rb][rb]   {$\Bvarphi$}
  \psfrag{phiD}  [rt][rt]   {$\Bvarphi \!=\! \bar \Bvarphi$}  
  \psfrag{qq}    [rb][rb]   {$\Bfrakq$}
  \psfrag{te}    [rb][rb]   {$T$}
  \psfrag{ql}    [lt][lt]   {$\Bfrakq^ l\!=\!\bar \Bfrakq^l$}
  \psfrag{tb}    [lt][lt]   {$T \!=\!\bar T$}
  \psfrag{defo}  [c][c]     {macro-motion field}
  \psfrag{long}  [c][c]     {micro-motion field}
  \psfrag{tem}   [c][c]     {thermal driving force}
  \includegraphics*[scale=0.5]{fields.eps}
  }
  \caption {Primary fields in thermomechanics of gradient-extended dissipative solids. At time $t$, the macro-motion field $\Bvarphi(\BX,t)$ is constrained by Dirichlet and Neumann boundary conditions $\Bvarphi = \bar \Bvarphi$ on $\partial \calB_\Bvarphi$ and $\BP \, \Bn_0 \ni  \bar \Bt$ on $\partial \calB_\Bt$. The long-range micro-motion field $\Bfrakq^l(\BX,t)$ is at time $t$ restricted by the  conditions $\Bfrakq^l = \bar \Bfrakq^l(\BX)$ on $\partial \calB_\Bfrakq$ and $ \BH^l \, \Bn_0 \ni \Bzero$ on $\partial \calB_H$. Finally, for a heat conducting solid the thermal driving force field $T(\BX,t)$ is at time $t$ constrained by the conditions $T = \bar T$ on $\partial \calB_T$ and $\Bq \cdot \Bn_0 = \bar q$ on $\partial \calB_q$.} 
\label{\LABEL}%         don't change
\end{figure}%         don't change


==> floats/mappings/fig.tex <==
\begin{figure}%         don't change

\centering
{
%
%  \footnotesize
  \psfrag{TXB}    [cc][cc][1][0] {$T_\BX \calB$}
  \psfrag{TxS}    [cc][cc][1][0] {$T_\Bx \calS$}
  \psfrag{TXsB}    [cc][cc][1][0] {$T_\BX^* \calB$}
  \psfrag{TxsS}    [cc][cc][1][0] {$T_\Bx^* \calS$}
  \psfrag{C}     [cc][cc][1][0] {$\BC$}
  \psfrag{g}  [cc][cc][1][0] {$\Bg$}  
  \psfrag{F}     [cc][cc][1][0] {$\BF$}
  \psfrag{Fd}     [cc][cc][1][0] {$\BF^{-T}$}
  \psfrag{Gp}     [cc][cc][1][0] {$\BG^p$}
  \psfrag{gp}     [cc][cc][1][0] {$\Bg^p$}
  \psfrag{aa}     [cc][cc] {{\footnotesize a)}}
  \psfrag{bb}     [cc][cc] {{\footnotesize b)}}
  \includegraphics*[scale=0.7]{mappings.eps}
  }
\caption {Geometry of additive plasticity. a) Definition of the total Hencky strain tensor $\Bvarepsilon = \frac{1}{2} \ln \BC$ in terms of the pull-back $\BC$ of the standard current metric $\Bg$. b) Definition of the plastic metric tensor $\BG^p$ on the reference configuration governing the plastic Hencky strain $\Bvarepsilon^p = \frac{1}{2} \ln \BG^p$ whose evolution is given by a local flow rule. Then, $\Bvarepsilon^e = \Bvarepsilon - \Bvarepsilon^p$ is the elastic strain measure entering the free energy function.
}
\label{\LABEL}%         don't change
\end{figure}%         don't change


==> floats/rheo/fig.tex <==
\begin{figure}%         don't change

\centering
{ \psfrag{q}[c][c] {$\frakq$}
  \psfrag{e}[c][c] {$\varepsilon$}
  \psfrag{s1}[l][l] {$\sigma_{ext}$}
  \psfrag{s2}[r][r] {$\sigma_{ext}$}
  \psfrag{H1}[c][c] {$H_1$}
  \psfrag{H2}[c][c] {$H_2$}
  \psfrag{E}[c][c] {$E, \alpha_T$}
  \psfrag{c}[c][c] {$C$}
  \psfrag{th}[c][c] {$\theta$}
%
  \includegraphics*[scale=0.9]{fig.eps}
  }
\caption {Rheological material element with internal thermoelastic and dissipative (viscous) mechanisms, loaded by an external stress $\sigma_{ext}(t)$. The time-discrete evolution of the material's state $(\varepsilon, \frakq, \eta)$ is described by  a finite sequence of incremental variational principles.
}

\label{\LABEL}%         don't change
\end{figure}%         don't change

